Learning Representations for Outlier Detection on a Budget

The problem of detecting a small number of outliers in a large dataset is an important task in many fields from fraud detection to high-energy physics. Two approaches have emerged to tackle this problem: unsupervised and supervised. Supervised approaches require a sufficient amount of labeled data and are challenged by novel types of outliers and inherent class imbalance, whereas unsupervised methods do not take advantage of available labeled training examples and often exhibit poorer predictive performance. We propose BORE (a Bagged Outlier Representation Ensemble) which uses unsupervised outlier scoring functions (OSFs) as features in a supervised learning framework. BORE is able to adapt to arbitrary OSF feature representations, to the imbalance in labeled data as well as to prediction-time constraints on computational cost. We demonstrate the good performance of BORE compared to a variety of competing methods in the non-budgeted and the budgeted outlier detection problem on 12 real-world datasets.

==> RWscores.tex <==
Diverse detection and scoring functions have been proposed including statistical approaches, PCA, and subspace analysis methods \cite{V. Barnett and T. Lewis. Outliers in Statistical Data, Wiley, 1994.; I. Jolliffe. Principal Component Analysis, Springer, 2002.;E. Muller, M. Schiffer, and T. Seidl. Statistical Selection of Relevant
Subspace Projections for Outlier Ranking. ICDE Conference,
pp, 434–445, 2011.;
Hoang Vu Nguyen, Vivekanand Gopalkrishnan, and Ira Assent. 2011. An unbiased distance-based outlier detection approach for high-dimensional data. In Proceedings of the 16th international conference on Database systems for advanced applications - Volume Part I (DASFAA'11), Jeffrey Xu Yu, Myoung Ho Kim, and Rainer Unland (Eds.), Vol. Part I. Springer-Verlag, Berlin, Heidelberg, 138-152. }.
 A large body of work is based on the analysis of distances and density around data points, e.g. via $k$NN distance or relative local density in LOF \cite{RamRasShi00,BreKriNgSan00}. Our method supports any such detectors that provide outlier scores.


I don't think it makes sense to define them all, that's just too much and not really relevant. Instead, give all citations at beginning of experiments, and state there  that this is just what we test, but any other scoring method would do as well.
\cite{RamRasShi00,AngPiz05,HauKaeFra04,BreKriNgSan00,SchZimKri14,TanCheFuChe02,JinTunHanWan06,KriKroSchZim09a,ZhaHutJin09,LatLazPok07,SchZimKri14a,KriSchZim08}.

